Video-XL: Extra-Long Vision Language Model for Hour-Scale Video Understanding

Long video understanding poses a significant challenge for current Multi-modal Large Language Models (MLLMs). Notably, the MLLMs are constrained by their limited context lengths and the substantial costs while processing long videos. Although several existing methods attempt to reduce visual tokens, their strategies encounter severe bottleneck, restricting MLLMs' ability to perceive fine-grained visual details. In this work, we propose Video-XL, a novel approach that leverages MLLMs' inherent key-value (KV) sparsification capacity to condense the visual input. Specifically, we introduce a new special token, the Visual Summarization Token (VST), for each interval of the video, which summarizes the visual information within the interval as its associated KV. The VST module is trained by instruction fine-tuning, where two optimizing strategies are offered. 1.Curriculum learning, where VST learns to make small (easy) and large compression (hard) progressively. 2. Composite data curation, which integrates single-image, multi-image, and synthetic data to overcome the scarcity of long-video instruction data. The compression quality is further improved by dynamic compression, which customizes compression granularity based on the information density of different video intervals. Video-XL's effectiveness is verified from three aspects. First, it achieves a superior long-video understanding capability, outperforming state-of-the-art models of comparable sizes across multiple popular benchmarks. Second, it effectively preserves video information, with minimal compression loss even at 16x compression ratio. Third, it realizes outstanding cost-effectiveness, enabling high-quality processing of thousands of frames on a single A100 GPU.

==> sec/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}


% background + importance


Inspired by the proliferation of large language models (LLMs)~\cite{openai2023gpt4, ChatGPT,touvron2023llama}, multimodal large language models (MLLMs)~\cite{li2023blip2, zhu2023minigpt4, liu2023visual_llava} have demonstrated remarkable capabilities in image understanding tasks by integrating visual encoders with LLMs and employing visual instruction tuning. Researchers are increasingly interested in transferring the knowledge from MLLMs to the video understanding domain, as video plays a crucial role in comprehending and interacting with the visual world.

% However, constructing video-based large language models (VideoLLMs) is challenging due to the complex and detailed nature of videos, which necessitates spatial-temporal joint modeling.

% 【一个直接的方式就是将视频切分成多图，将mllms的多图能力泛化到视频域上。然而他们仅仅能处理短视频不能处理长视频，这主要是长视频会产生大量视觉token。一方面超过了语言模型窗口长度，另一方面LLM计算复杂度超过了显存限制。（举例子）】【最近一些工作尝试解决这个问题。他们采用预先压缩的方式，设计模块在LLM之前对视觉token的数量进行压缩；然而，由于压缩带来的损失，他们无法对长序列中的细节信息进行有效的信息保留。（展开：subaction, 关键情节。。）】【跟他们不同，LOngva不做压缩扩展了语言模型上下文，然而他依旧面临显存消耗的问题。（展开）】

% Technical Challenges 1.VLM short (cost and data); 2. concurrent LVU -> info bottleneck


Constructing video-based large language models (VideoLLMs) is non-trivial due to spatial-temporal joint modeling. A straightforward approach is to insert additional learnable modules~\cite{videollama,li2024mvbench,videollava} into image-based MLLMs to capture temporal information by feeding them sequences of frames extracted from videos. (i) The massive number of visual tokens generated by the visual encoder may exceed the context window length of LLMs, leading to impractical computational complexity and memory costs; (ii) There is a scarcity of high-quality long video datasets, which fail to provide effective supervision signals. Some current works~\cite{liu2024world,longva} attempt to directly extend the context size of LLMs to accommodate more visual tokens. However, they still overlook the computational costs incurred during the inference. As illustrated in Figure 1, nearly all VideoLLMs can process no more than 1,000 frames on a single A100 80GB  GPU. To address this challenge, various precompression mechanisms~\cite{maaz2023videochatgpt,llamavid,weng2024longvlm,moviechat2023,malmm2024} are designed for dropping visual tokens before inputting them into the LLM. While these approaches can handle longer videos, they often encounter inevitable information bottlenecks due to the reduction of visual signals.

% To address these challenges, current work leverages the temporal and spatial redundancy of long videos by designing precompression mechanisms~\cite{maaz2023videochatgpt,llamavid,weng2024longvlm,moviechat2023,malmm2024} for visual tokens before inputting them into the LLM. While these approaches can handle longer videos, they often encounter inevitable information bottlenecks due to the reduction of visual tokens.
% fine-grained information understanding and long-term temporal connections. The reduction in visual tokens inevitably results in the loss of key details, making it difficult for models to capture subtle actions, character expressions, and the order of events. 
% In contrast to the aforementioned methods, some works~\cite{liu2024world,longva} attempt to directly extend the context size of LLMs to accommodate more visual tokens. However, they often overlook the computational costs incurred during the inference stage. As illustrated in Figure 1, nearly all VideoLLMs can process no more than 1,000 frames on a single A100 80GB  GPU.  

 



% 我们尝试回答这个问题：能否不在LLM前设计额外的压缩模块，而是利用LLM的固有能力，便可以使videollms在大量token中即保持细节，同时具有较小的内存开销。为了探究这个问题，我们，首先探究了LLM的两个特性：（1）拥有处理视觉序列的能力（展开）；（2）压缩的能力（kv cache压缩）

%% Intuitive: LLM work as a strong info compressor  
% nlp: kv comkpression -> strong potential 

In this paper, we aim to address the question: \textit{ Can we find an optimal solution for VideoLLMs to achieve effective visual information compression?} Instead of designing extra modules, we approach this question by identifying two features of LLMs.

% Is it possible for VideoLLMs to achieve visual information compression by solely leveraging the inherent capabilities of LLMs, without the need for additional compression modules? }
% effective long video understanding while maintaining reasonable memory overhead, by solely leveraging the inherent capabilities of LLMs, without the need for additional compression modules?} We approach this question by identifying two  features of LLMs:

\noindent\textbf{Visual modeling}: Although LLMs are primarily trained in the natural language domain, they exhibit remarkable potential beyond linguistic applications.  ~\cite{pang2023frozen,wang2024adapting} have demonstrated that pre-trained LLM transformer blocks can perceive informative visual tokens and posses image understanding capabilities.


% For instance, ~\cite{pang2023frozen} found that pre-trained LLM transformer blocks can discern informative visual tokens. Similarly, ~\cite{wang2024adapting} demonstrated that decoder-only transformers possess image understanding capabilities with only minor modifications to the attention masks.


\noindent\textbf{Context compression}: To achieve computational efficiency, numerous approaches~\cite{chevalier2023adapting,zhang2024soaring,jiang2023llmlingua} have focused on compressing raw input into more compact representations by modifying the workflow of LLM, thereby reducing both the computational cost of inference and the memory overhead associated with the key-value (KV) cache. 


% This strategy allows the generation process to be conditioned on a shorter context, thereby reducing both the computational cost of inference and the memory overhead associated with the key-value (KV) cache. Additionally, it facilitates the processing of longer inputs than what the LLM's built-in context window would typically allow. 


% 基于以上发现，我们提出了VideoXL，仅仅利用llm天然的能力去实现精确长视频理解，而没有在llm前建立额外的压缩模块。具体来说，为了实现细粒度的信息理解，我们将视觉长序列划分为多个长度不一样的chunks（每个chunk长度小于语言模型的窗口长度）, 并让LLM按顺序encode他们。为了实现长时序的联系，我们提出了vst token， 将每个chunk中常规token的特征蒸馏到vst token 的kvcache中去。具体来说，每个chunk会进一步划分为a个单位，vst将会被交互式的插入。 随着LLM逐渐处理每个chunk，raw token的activations会被抛弃，vst的activationsh会被累积并重复用于编码下一个chunk。 VideoXL具有以下的highlights：（1）实现细粒度的信息理解，因为LLM每次只详细看了视频的一小部分，并且关键信息可以被VST保留；（2）实现长距离时序关联，通过存储和复用vst cache实现。（3）可以处理远超过语言模型上下文的视觉序列并且保证较低的计算复杂度，因为每个chunk的self attention只作用于前序更短的上下文中。
% 同时，我们进一步挖掘了vst的attention scope对长视频理解的影响，发现vst难以学习上下文不一致的视频内容；因此我们根据无监督语义分割算法自动划分长度不一样的chunk，确保每个chunk中是语义一致的视觉内容。受到课程学习思想的启发，我们并非对每个chunk设置固定的压缩比，而是随机设计压缩比，并且随着训练step的增加对压缩比进行逐渐增大，从而加快模型的收敛速度。（压缩机制训练机制）


% 修改 %%% 强调challenge
%%% 强调视觉
% 基于以上发现，我们提出了VideoXL，仅仅利用llm天然的能力去实现精确长视频理解，而没有在llm前建立额外的压缩模块。首先，我们将视觉长序列划分为多个细粒度的chunks, 然后在每个chunk中设立vst， 将常规token的特征蒸馏到vst token 的kvcache中去。同时，为了防止细节信息在压缩中的损失，我们设计了无监督语义分割算法来自适应切分chunk，确保每个chunk中是完整的语义片段。随着LLM逐渐处理每个chunk，raw token的activations会被抛弃，vst的activationsh会被累积并重复用于编码下一个chunk。最后，受到课程学习思想的启发，我们并非对每个chunk设置固定的压缩比，而是随机设计压缩比，并且随着训练step的增加对压缩比进行逐渐增大，从而加快模型的收敛速度。 VideoXL具有以下的highlights：（1）实现细粒度的信息理解，因为LLM每次只详细看了视频的一小部分，并且dc设计使得关键信息可以被VST保留；（2）实现长距离时序关联，通过存储和复用vst cache实现。（3）可以处理远超过语言模型上下文的视觉序列并且保证较低的计算复杂度，因为每个chunk的self attention只作用于前序更短的上下文中。

%

Based on the above observations, we intuitively argue LLM itself can work as a strong visual information condensor, thus propose our Video-XL. Similar to the popular visual instruction tuning pipeline, Video-XL involves only minor modifications to the LLM architecture. Specifically, we split long visual tokens into multiple chunks of shorter lengths, then introduce Visual Summarization Tokens (VSTs) to the original visual context, distilling the raw activations of visual latents (i.e., keys and values in the self-attention module) into VST activations.  As each chunk is encoded progressively by the LLM, the activations of the raw visual tokens are discarded, while the VST activations are accumulated and reused for encoding subsequent chunks. 

% propose Video-XL. Instead of incorporating an extra compression module \textbf{before the LLM}, we leverage the \textbf{inherent capacity of the LLM} to compress massive visual tokens. Similar to the popular visual instruction tuning pipeline, Video-XL involves only minor modifications to the LLM architecture. Specifically, we split long visual tokens into multiple chunks of shorter lengths. We then introduce Visual Summarization Tokens (VSTs) to the original visual context, distilling the raw activations of visual latents (i.e., keys and values in the self-attention module) into VST activations.  As each chunk is encoded progressively by the LLM, the activations of the raw visual tokens are discarded, while the VST activations are accumulated and reused for encoding subsequent chunks. 

% 压缩机制的优化：视觉跟语言之间的diff，信息密度时序非均衡 -> 动态chunk分配，训练方式优化（课程学习）




Meanwhile, directly compressing visual context into VSTs in a chunk still incurs fine-grained information loss. Compared to natural language, visual information intensity is imbalanced in the temporal dimension. To this end, we first implement a temporal semantic segmentation approach to adaptively tailor each chunk, ensuring that each chunk contains intact semantic segments. Then we propose a curriculum learning-based training process that establishes a variable compression ratio for each chunk, beginning with lower ratios and progressively increasing them as training advances.



% In summary, Video-XL has the following highlights: (i) It achieves fine-grained information understanding by focusing on small segments of long video sequences and compactly preserving features in VSTs; (ii) It establishes long-term temporal connections by storing and reusing the KV caches of VSTs; (iii) It facilitates the processing of longer videos, with token counts exceeding the LLM’s built-in context window, while maintaining reasonable computational costs, as the generation process is conditioned on a shorter context.



% 除了VideoXL的设计，我们还探究了不同类型多模态数据对长视频理解的影响。通过利用视觉统一编码形式，我们发现单图，多图，视频对长视频理解不同方面的贡献。具体而言，单图提升模型的细节空间感知能力；多图数据使模型分辨输入内容的差异；视频数据提升长序列检索能力；我们还从训练效率和效果层面分析了不同类型数据配比的影响；最后，为了弥补多跳推理能力，我们提出了vico数据集。

%% knowledge transfer+ data （想从两个层面来说；一个是单图和多图的知识迁移->统一的视觉编码机制，另一个是在视频数据内部探究在有限的视频时长内最适合泛化到长视频的任务形式）

Beyond the design of Video-XL, we investigate the  \textit{knowledge transfer phenomenon} in long video understanding. On one hand, leveraging unified visual encoding, we observe that not only can video data but also single images and multiple images contribute to long video understanding in various capacities, thereby alleviating the current scarcity of long video training data. We also analyze the impact of different data type ratios on training efficiency and effectiveness. On the other hand, we explore the most suitable task forms within the limited duration of video data that generalize effectively to longer videos. We introduce a new video dataset named Visual Clue Ordering (VICO), which contains 20k high-quality long video question-answer pairs to enhance the model's multi-detail retrieval capabilities.

% different multimodal data (single images, multi-images, and videos) contribute to long video understanding in different capacities. We also analyze the impact of different data type ratios on training efficiency and effectiveness. Lastly, we introduce a long video dataset named VIsual Clue Ordering (VICO) to enhance the model's multi-detail retrieval capabilities.


% explore how different multimodal data types (single images, multi-images, and videos) contribute to long video understanding. Specifically, the unified visual encoding representation allows single images to enhance the model's detail perception capabilities. Multi-image data enable the model to distinguish differences in input content, while video data enhances the ability to retrieve key information from long sequences. We also analyze the impact of different data type ratios on training efficiency and effectiveness. Lastly, we introduce a long video dataset named VIsual Clue Ordering (VICO) to enhance the model's multi-detail retrieval capabilities.




% main contribution:
% (1) 利用llm天然能力实现准确长视频理解，取得两个目标同时保持计算效率
% （2）videoxl 的techniqal design， 动态chunk以及训练方式
% （3）从数据角度rethink了不同多模态数据对lvu的影响以及进一步探究数据配比
% （4） 实验结果：（i）general 效果：长视频上sota，短视频上也不错, 图像也能做；(ii) 长且effiency，needle实验


Overall, our main contributions are threefold:

(i) We introduce Video-XL, which harnesses the inherent capacity of the LLM to compress visual tokens. To better maintain fine-grained information, we implement a semantic-aware chunk tailoring mechanism and propose a curriculum learning-based training process with random compression ratio control. 

(ii) We investigate the phenomenon of knowledge transfer in long video understanding by leveraging information from single images and multiple images, and by proposing a new video dataset, VICO, which enhances the model's generalization to longer videos.


% rethink long video understanding from a data-centric perspective by exploring how different multi-modal data contribute to this task and uncovering their optimal data matching.

(iii) Video-XL demonstrates leading performance on popular long video benchmarks and achieves promising results in short video and image understanding tasks. It strikes an excellent balance between efficiency and effectiveness, processing 2048 frames on a single A100-80GB GPU while attaining nearly 95\% accuracy in the Needle-in-a-Haystack~\cite{longva} evaluation.

%-------------------------------------------------------------------------
\section{Related work}

\subsection{LLM-based short video understanding}
Recent advancements in Multimodal Language Models (MLLMs)~\cite{li2022blip,li2023blip2,dai2023instructblip,liu2023visual_llava,zhu2023minigpt4} have significantly improved performance in image understanding tasks. Consequently, numerous studies have sought to adapt MLLMs for the video understanding domain by incorporating additional learnable modules between the visual encoder and the LLM to capture temporal information. For instance, VideoChat-GPT~\cite{maaz2023videochatgpt} and Valley~\cite{luo2023valley} implement spatial and temporal pooling over visual tokens to extract key visual representations. ST-LLM~\cite{stllm}, VideoChat~\cite{li2023videochat}, and VideoChat2~\cite{li2024mvbench} utilize Q-Former to effectively model temporal relationships, while Video-LLaMA~\cite{videollama} establishes dual Q-Former branches to facilitate video and audio interaction. Additionally, Chat-UniVi~\cite{chatunivi} employs a set of dynamic visual tokens to uniformly represent both images and videos. Despite the promising results these approaches have achieved in short video understanding, they remain limited in their effectiveness for long video comprehension.



\subsection{LLM-based long video understanding}
To address the challenge posed by the thousands of visual tokens generated by long videos, current research has focused on designing pre-compression mechanisms prior to LLM processing. For instance, MovieChat~\cite{moviechat2023} and MA-LMM~\cite{malmm2024} implement effective memory modules that comprise a long-term memory bank to capture historical information and a short-term memory bank to cache current conditions, resulting in more accurate and consistent predictions over time for long videos. LLmMA-VID~\cite{llamavid} represents each frame to only two tokens by employing a context attention module. To enhance the capacity for long context modeling, LongVLM~\cite{weng2024longvlm} introduces a token-merging module to aggregate local features from short segments along with global context features, while Video-CCAM~\cite{fei2024videoccam} incorporates cross-attention calculations using causal cross-attention masks. Despite the introduction of these compression modules, which show promise for long video understanding, the reduction in visual tokens inevitably leads to information loss, posing challenges for fine-grained information comprehension and maintaining long-term temporal connections.


Unlike the aforementioned methods, LWM~\cite{liu2024world} gradually extends the context size by optimizing the implementation of RingAttention~\cite{liu2024blockwise}, while LongVA~\cite{longva} directly expands the LLM's context length to accommodate longer visual sequences. Other approaches focus on improving training methods~\cite{longvila} or LLM architecture~\cite{wang2024longllava}, but they fail to effectively address the computational and memory challenges during inference.

\section{Method}


\subsection{Overview}
% 结构跟llava类似，由visual encder，projector和llm组成，通过visual instruction tuning 方法训练；不同的是，videoxl在训练时设计了统一的视觉编码机制以利用不同类型的多模态数据（3.2）； 同时为了压缩大量视觉token，我们修改了LLM的工作流，使其可以无损压缩视觉token（3.3）。最后我们介绍了videoxl的training pipeline(3.4)

Similar to traditional MLLMs, Video-XL comprises a visual encoder, a visual language projector, and an LLM, trained using a visual instruction tuning approach. However, we design a unified visual encoding mechanism to represent various multimodal data in a common space (see Section~\ref{sec:visual}). Furthermore, we modify the LLM workflow to effectively compress large visual tokens to achieve promising long video understanding (see Section~\ref{sec:llm}). Finally, we briefly illustrate our training pipeline in Section~\ref{sec:training_pipeline}. 


\subsection{Visual Encoding}
\label{sec:visual}
% 如何把不同多模态数据统一；如何消除不同数据的gap； 细节（图像encoder还是视频encoder,projector设计，token数量）



% 设计一套强大的视觉编码机制对lvu至关重要，首先在于视觉编码器的选择。尽管目前出现了很多视频foundationmodel，但他们难以处理任意长度的视频；另外clip已经在很多视频理解任务中展现出了强大的性能；其次，很多工作尝试将各种多模态数据统一编码，然而不同类型数据之间存在的gap会损失lvu的性能。

Designing an effective visual encoding mechanism is crucial for long video understanding. First, the choice of visual encoder is essential. While some video foundation models~\cite{bertasius2021space,li2023unmasked} have been proposed, they are unable to handle arbitrary frames, whereas CLIP~\cite{radford2021clip} have demonstrated strong potential in various video down-stream tasks~\cite{conti2024vocabulary,mi2023clif}. Furthermore, video-only encoding is insufficient due to the scarcity of video training data. Although many studies~\cite{li2024llavaonevision, internvl, wang2024qwen2vl} have demonstrated the coexistence of MLLMs that support different multimodal data (single images, multi-images, and video), the disparity between these data types still results in decreased performance in long video understanding.

Thus, we opt for CLIP-ViT-L as our visual encoder and encode different mutli-modal data into a unified represeantion  motivated by ~\cite{longva}. Specifically, given a single image , we divide it into multiple patches, each with a resolution of $336 \times 336$ which will be encoded by CLIP seperately,


resulting $(h//336) \times (w//336) \times M$ tokens, where $h$ and $w$ is the original size of image. While a multi-image or video contains N frames  
 



An N-frame video is treated as an image of size 336 × (336 × N), divided into
N grids where each grid corresponds to a video frame.

for multi-images or videos, we input frames with a resolution of $336 \times 336$ directly into CLIP. For single images, we divide them into patches, each with a resolution of $336 \times 336$, and then feed these patches into CLIP. Consequently, an N-frame video or N-patch image is encoded into $N \times M$ tokens, where $M$ represents the number of tokens per image. The patch-splitting method follows the approach described in ~\cite{longva}. For video processing, we sample one frame per second for videos shorter than 128 frames. For longer videos, we uniformly sample 128 frames.




UniRes allows us to unifiedly encode videos as well. A video is treated as an extended image where
each frame is considered as an image grid.

% 


\subsection{LLM Compressing}
\label{sec:llm}

\subsection{Training Pipeline}
\label{sec:training_pipeline}


\section{Knowledge Transfer Phenomenon}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
